A First Look at Android Applications in Google Play related to Covid-19

Due to the convenience of access-on-demand to information and business solutions, mobile apps have become an important asset in the digital world. In the context of the Covid-19 pandemic, app developers have joined the response effort in various ways by releasing apps that target different user bases (e.g., all citizens or journalists), offer different services (e.g., location tracking or diagnostic-aid), provide generic or specialized information, etc. While many apps have raised some concerns by spreading misinformation or even malware, the literature does not yet provide a clear landscape of the different apps that were developed. In this study, we focus on the Android ecosystem and investigate Covid-related Android apps. In a best-effort scenario, we attempt to systematically identify all relevant apps and study their characteristics with the objective to provide a First taxonomy of Covid-related apps, broadening the relevance beyond the implementation of contact tracing. Overall, our study yields a number of empirical insights that contribute to enlarge the knowledge on Covid-related apps: (1) Developer communities contributed rapidly to the Covid-19, with dedicated apps released as early as January 2020; (2) Covid-related apps deliver digital tools to users (e.g., health diaries), serve to broadcast information to users (e.g., spread statistics), and collect data from users (e.g., for tracing); (3) Covid-related apps are less complex than standard apps; (4) they generally do not seem to leak sensitive data; (5) in the majority of cases, Covid-related apps are released by entities with past experience on the market, mostly official government entities or public health organizations.

==> leaks.tex <==
\section{Details of leaks found by FlowDroid-IccTA}
\label{appendix:leaks}

Below we present the different potential leaks that were found by FlowDroid-IccTA.

\subsection{Leaks in app com.bloomreality.sodi}
\begin{flushleft}
\begin{itemize}
    \item Found a flow to sink virtualinvoke \$r0.$<$android.content.Context: android.content.Intent registerReceiver(android.content.BroadcastReceiver,android.content.IntentFilter)$>$(\$r5, \$r4) on line 39, from the following sources:
    \begin{itemize}
        \item \$r1 := @parameter0: android.content.Context (in $<$mono.MonoRuntimeProvider: void attachInfo(android.content.Context,android.content.pm.ProviderInfo)$>$)
                on Path [\$r1 := @parameter0: android.content.Context, staticinvoke $<$mono.MonoPackageManager: void LoadApplication(android.content.Context,android.content.pm.ApplicationInfo,java\-.lang.String[])$>$(\$r1, \$r3, \$r5), virtualinvoke \$r0.$<$android.content.Context: android.content\-.Intent registerReceiver(android.content.BroadcastReceiver,android.content.IntentFilter\-)$>$(\$r5, \$r4)]
    \end{itemize}
\end{itemize}


\subsection{Leaks in app br.gov.datasus.guardioes}

\begin{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int w(java.lang.String,java.lang.String)$>$(\$r0, \$r2) on line 436, from the following sources:
    \begin{itemize}
	\item  \$r3 = virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: android.content.Intent getIntent()$>$() (in $<$org.apache.cordova.CordovaActivity: void loadConfig()$>$)
		on Path [\$r3 = virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: android.content.Intent getIntent()$>$(), \$r4 = virtualinvoke \$r3.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), virtualinvoke \$r2.$<$org.apache.cordova.CordovaPreferences: void setPreferencesBundle(android.os.Bundle)$>$(\$r4), \$r0.$<$org.apache.cordova.CordovaPreferences: android.os.Bundle preferencesBundleExtras$>$ = \$r1, \$r0 := @this: org.apache.cordova.CordovaPreferences, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaPreferences preferences$>$, return, return, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void onResume()$>$(), staticinvoke $<$com.dynatrace.android.callback.Callback: void onResume(android.app.Activity)$>$(\$r0), virtualinvoke \$r2.$<$com.dynatrace.android.app.LcCallbacks: void onActivityResume(android.app.Activity)$>$(\$r0), virtualinvoke \$r3.$<$com.dynatrace.android.app.LcContext: void enterAction(android.app.Activity,com.dynatrace.android.agent.data.LcData\-Constants\$LcState)$>$(\$r1, \$r2), \$r9 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r10 = virtualinvoke \$r9.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), virtualinvoke \$r11.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r10), \$r12 = virtualinvoke \$r11.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r13 = specialinvoke \$r0.$<$com.dynatrace.android.app.LcContext: com.dynatrace.android.agent.DTXAutoAction getAutoUserAction(java.lang.String,long)$>$(\$r12, -1L), \$r2 = staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction createAutoAction(java.lang.String,long)$>$(\$r1, \$l0), \$r0 = staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction createAutoAction(java.lang.String)$>$(\$r1), specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXAutoAction: void $<$init$>$(java.lang.String)$>$(\$r1), specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: void $<$init$>$(java.lang.String,com.dynatrace.android.agent.EventType,long)$>$(\$r1, \$r3, 0L), specialinvoke \$r0.$<$com.dynatrace.android.agent.CustomSegment: void $<$init$>$(java.lang.String,int,com.dynatrace.android.agent.EventType,long)$>$(\$r1, 5, \$r2, \$l0), specialinvoke \$r0.$<$com.dynatrace.android.agent.CustomSegment: void setName(java.lang.String)$>$(\$r1), \$r0.$<$com.dynatrace.android.agent.CustomSegment: java.lang.String mName$>$ = \$r1, return, return, return, return, staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction swapGaua(com.dynatrace.android.agent.DTXAutoAction)$>$(\$r0), $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction theAutoAction$>$ = \$r1, virtualinvoke \$r48.$<$com.adobe.phonegap.push.FCMService: void onMessageReceived(com.google.firebase.messaging.RemoteMessage)$>$(\$r51), specialinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: void showNotificationIfPossible(android.content.Context,android.os.Bundle)$>$(\$r13, \$r5), virtualinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: void createNotification(android.content.Context,android.os.Bundle)$>$(\$r1, \$r2), specialinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: void setNotificationMessage(int,android.os.Bundle,android.support.v4.app.Notification\-Compat\$Builder)$>$(\$i0, \$r2, \$r13), \$r15 = virtualinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: android.graphics.Bitmap getBitmapFromURL(java.lang.String)$>$(\$r4), staticinvoke $<$com.dynatrace.android.callback.Callback: void openConnection(java.net.URLConnection)$>$(\$r3), staticinvoke $<$com.dynatrace.android.callback.CallbackCore: com.dynatrace.android.callback.CbWebReqTracker addConnection(java.net.HttpURLConnection,boolean)$>$(\$r1, 1), \$r7 = staticinvoke $<$com.dynatrace.android.callback.CallbackCore\$ConnRegistration: com.dynatrace.android.callback.CbWebReqTracker access\$100(com.dynatrace.android.callback.CallbackCore\$ConnRegistration)$>$(\$r1), \$r1 = specialinvoke \$r0.$<$com.dynatrace.android.callback.CallbackCore\$ConnRegistration: com.dynatrace.android.callback.CbWebReqTracker register()$>$(), \$r4 = staticinvoke $<$com.dynatrace.android.callback.CallbackCore: com.dynatrace.android.callback.CbWebReqTracker access\$300(java.net.HttpURLConnection)$>$(\$r2), \$r1 = staticinvoke $<$com.dynatrace.android.callback.CallbackCore: com.dynatrace.android.callback.CbWebReqTracker registerConn(java.net.HttpURLConnection)$>$(\$r0), \$r10 = staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction getAutoAction()$>$(), r0 = $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction theAutoAction$>$, return r0, \$i0 = virtualinvoke \$r10.$<$com.dynatrace.android.agent.DTXAutoAction: int tagRequest(java.net.HttpURLConnection)$>$(\$r0), \$i0 = specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: int tagRequest(java.net.HttpURLConnection)$>$(\$r1), \$i0 = virtualinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: int getPreconditions()$>$(), \$i0 = specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: int getPreconditions()$>$(), \$r3 = virtualinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: java.lang.String getName()$>$(), r1 = \$r0.$<$com.dynatrace.android.agent.CustomSegment: java.lang.String mName$>$, return r1, \$r2[0] = \$r3, \$r3 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("Maximum depth of actions reached (10). Discarding creation of \'\%s\'", \$r2), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogW(java.lang.String,java.lang.String)$>$(\$r1, \$r3), virtualinvoke \$r1.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r2), \$r2 = virtualinvoke \$r1.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int w(java.lang.String,java.lang.String)$>$(\$r0, \$r2)]
		
	\item  \$r1 := @parameter0: android.os.Bundle (in $<$br.gov.datasus.guardioes.MainActivity: void onCreate(android.os.Bundle)$>$)
		on Path [\$r1 := @parameter0: android.os.Bundle, specialinvoke \$r0.$<$org.apache.cordova.CordovaActivity: void onCreate(android.os.Bundle)$>$(\$r1), virtualinvoke \$r5.$<$org.apache.cordova.CordovaInterfaceImpl: void restoreInstanceState(android.os.Bundle)$>$(\$r1), \$r1 = virtualinvoke \$r1.$<$android.os.Bundle: android.os.Bundle getBundle(java.lang.String)$>$("plugin"), \$r0.$<$org.apache.cordova.CordovaInterfaceImpl: android.os.Bundle savedPluginState$>$ = \$r1, \$r0 := @this: org.apache.cordova.CordovaInterfaceImpl, \$r5 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaInterfaceImpl cordovaInterface$>$, return, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void onStart()$>$(), staticinvoke $<$com.dynatrace.android.callback.Callback: void onStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r2.$<$com.dynatrace.android.app.LcCallbacks: void onActivityStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r3.$<$com.dynatrace.android.app.LcContext: void enterAction(android.app.Activity,com.dynatrace.android.agent.data.LcData\-Constants\$LcState)$>$(\$r1, \$r2), \$r9 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r10 = virtualinvoke \$r9.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), virtualinvoke \$r11.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r10), \$r12 = virtualinvoke \$r11.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r13 = specialinvoke \$r0.$<$com.dynatrace.android.app.LcContext: com.dynatrace.android.agent.DTXAutoAction getAutoUserAction(java.lang.String,long)$>$(\$r12, -1L), \$r2 = staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction createAutoAction(java.lang.String,long)$>$(\$r1, \$l0), \$r0 = staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction createAutoAction(java.lang.String)$>$(\$r1), specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXAutoAction: void $<$init$>$(java.lang.String)$>$(\$r1), specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: void $<$init$>$(java.lang.String,com.dynatrace.android.agent.EventType,long)$>$(\$r1, \$r3, 0L), specialinvoke \$r0.$<$com.dynatrace.android.agent.CustomSegment: void $<$init$>$(java.lang.String,int,com.dynatrace.android.agent.EventType,long)$>$(\$r1, 5, \$r2, \$l0), specialinvoke \$r0.$<$com.dynatrace.android.agent.CustomSegment: void setName(java.lang.String)$>$(\$r1), \$r0.$<$com.dynatrace.android.agent.CustomSegment: java.lang.String mName$>$ = \$r1, return, return, return, return, staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction swapGaua(com.dynatrace.android.agent.DTXAutoAction)$>$(\$r0), $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction theAutoAction$>$ = \$r1, virtualinvoke \$r48.$<$com.adobe.phonegap.push.FCMService: void onMessageReceived(com.google.firebase.messaging.RemoteMessage)$>$(\$r51), specialinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: void showNotificationIfPossible(android.content.Context,android.os.Bundle)$>$(\$r13, \$r5), virtualinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: void createNotification(android.content.Context,android.os.Bundle)$>$(\$r1, \$r2), specialinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: void setNotificationMessage(int,android.os.Bundle,android.support.v4.app.Notification\-Compat\$Builder)$>$(\$i0, \$r2, \$r13), \$r15 = virtualinvoke \$r0.$<$com.adobe.phonegap.push.FCMService: android.graphics.Bitmap getBitmapFromURL(java.lang.String)$>$(\$r4), staticinvoke $<$com.dynatrace.android.callback.Callback: void openConnection(java.net.URLConnection)$>$(\$r3), staticinvoke $<$com.dynatrace.android.callback.CallbackCore: com.dynatrace.android.callback.CbWebReqTracker addConnection(java.net.HttpURLConnection,boolean)$>$(\$r1, 1), \$r7 = staticinvoke $<$com.dynatrace.android.callback.CallbackCore\$ConnRegistration: com.dynatrace.android.callback.CbWebReqTracker access\$100(com.dynatrace.android.callback.CallbackCore\$ConnRegistration)$>$(\$r1), \$r1 = specialinvoke \$r0.$<$com.dynatrace.android.callback.CallbackCore\$ConnRegistration: com.dynatrace.android.callback.CbWebReqTracker register()$>$(), \$r4 = staticinvoke $<$com.dynatrace.android.callback.CallbackCore: com.dynatrace.android.callback.CbWebReqTracker access\$300(java.net.HttpURLConnection)$>$(\$r2), \$r1 = staticinvoke $<$com.dynatrace.android.callback.CallbackCore: com.dynatrace.android.callback.CbWebReqTracker registerConn(java.net.HttpURLConnection)$>$(\$r0), \$r10 = staticinvoke $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction getAutoAction()$>$(), r0 = $<$com.dynatrace.android.agent.DTXAutoAction: com.dynatrace.android.agent.DTXAutoAction theAutoAction$>$, return r0, \$i0 = virtualinvoke \$r10.$<$com.dynatrace.android.agent.DTXAutoAction: int tagRequest(java.net.HttpURLConnection)$>$(\$r0), \$i0 = specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: int tagRequest(java.net.HttpURLConnection)$>$(\$r1), \$i0 = virtualinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: int getPreconditions()$>$(), \$i0 = specialinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: int getPreconditions()$>$(), \$r3 = virtualinvoke \$r0.$<$com.dynatrace.android.agent.DTXActionImpl: java.lang.String getName()$>$(), r1 = \$r0.$<$com.dynatrace.android.agent.CustomSegment: java.lang.String mName$>$, return r1, \$r2[0] = \$r3, \$r3 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("Maximum depth of actions reached (10). Discarding creation of \'\%s\'", \$r2), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogW(java.lang.String,java.lang.String)$>$(\$r1, \$r3), virtualinvoke \$r1.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r2), \$r2 = virtualinvoke \$r1.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int w(java.lang.String,java.lang.String)$>$(\$r0, \$r2)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r4, \$r6) on line 17, from the following sources:
\begin{itemize}
	\item  \$r2 := @parameter1: android.content.Intent (in $<$com.adobe.phonegap.push.BackgroundActionButtonHandler: void onReceive(android.content.Context,android.content.Intent)$>$)
		on Path [\$r2 := @parameter1: android.content.Intent, \$r3 = virtualinvoke \$r2.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), virtualinvoke \$r5.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.Object)$>$(\$r3), \$r6 = virtualinvoke \$r5.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r4, \$r6)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r5, \$r7) on line 20, from the following sources:
\begin{itemize}
	\item  \$r3 := @parameter1: android.content.Intent (in $<$com.adobe.phonegap.push.PushDismissedHandler: void onReceive(android.content.Context,android.content.Intent)$>$)
		on Path [\$r3 := @parameter1: android.content.Intent, \$i0 = virtualinvoke \$r3.$<$android.content.Intent: int getIntExtra(java.lang.String,int)$>$("notId", 0), virtualinvoke \$r6.$<$java.lang.StringBuilder: java.lang.StringBuilder append(int)$>$(\$i0), \$r7 = virtualinvoke \$r6.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r5, \$r7)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int e(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r0, \$r3, \$r1) on line 426, from the following sources:
\begin{itemize}
	\item  \$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$() (in $<$com.dynatrace.android.agent.comm.CommHandler: java.net.HttpURLConnection openConnection(java.net.URL)$>$)
		on Path [\$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$(), \$r5 = (java.net.HttpURLConnection) \$r4, return \$r5, \$i0 = virtualinvoke \$r6.$<$java.net.HttpURLConnection: int getResponseCode()$>$(), specialinvoke r31.$<$com.dynatrace.android.agent.comm.HttpResponse: void $<$init$>$(int,java.lang.String,java.lang.String,java.util.Map)$>$(\$i0, \$r1, \$r2, \$r8), \$r0.$<$com.dynatrace.android.agent.comm.HttpResponse: int responseCode$>$ = \$i0, \$r0 := @this: com.dynatrace.android.agent.comm.HttpResponse, \$r24 = r31, return \$r24, specialinvoke \$r6.$<$com.dynatrace.android.agent.comm.InvalidResponseException: void $<$init$>$(java.lang.String,com.dynatrace.android.agent.comm.HttpResponse)$>$(\$r4, \$r5), \$r0.$<$com.dynatrace.android.agent.comm.InvalidResponseException: com.dynatrace.android.agent.comm.HttpResponse response$>$ = \$r2, return, throw \$r6, staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogE(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r1, "time sync request failed", \$r10), staticinvoke $<$android.util.Log: int e(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r0, \$r3, \$r1)]

	\item  \$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$() (in $<$com.dynatrace.android.agent.comm.CommHandler: java.net.HttpURLConnection openConnection(java.net.URL)$>$)
		on Path [\$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$(), \$r6 = (javax.net.ssl.HttpsURLConnection) \$r4, return \$r6, \$i0 = virtualinvoke \$r6.$<$java.net.HttpURLConnection: int getResponseCode()$>$(), specialinvoke r31.$<$com.dynatrace.android.agent.comm.HttpResponse: void $<$init$>$(int,java.lang.String,java.lang.String,java.util.Map)$>$(\$i0, \$r1, \$r2, \$r8), \$r0.$<$com.dynatrace.android.agent.comm.HttpResponse: int responseCode$>$ = \$i0, \$r0 := @this: com.dynatrace.android.agent.comm.HttpResponse, \$r24 = r31, return \$r24, specialinvoke \$r6.$<$com.dynatrace.android.agent.comm.InvalidResponseException: void $<$init$>$(java.lang.String,com.dynatrace.android.agent.comm.HttpResponse)$>$(\$r4, \$r5), \$r0.$<$com.dynatrace.android.agent.comm.InvalidResponseException: com.dynatrace.android.agent.comm.HttpResponse response$>$ = \$r2, return, throw \$r6, staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogE(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r1, "time sync request failed", \$r10), staticinvoke $<$android.util.Log: int e(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r0, \$r3, \$r1)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1) on line 401, from the following sources:
\begin{itemize}
	\item  \$d0 = virtualinvoke \$r0.$<$android.location.Location: double getLongitude()$>$() (in $<$com.dynatrace.android.agent.Core: int setGpsLocation(android.location.Location)$>$)
		on Path [\$d0 = virtualinvoke \$r0.$<$android.location.Location: double getLongitude()$>$(), \$r3 = staticinvoke $<$java.lang.Double: java.lang.Double valueOf(double)$>$(\$d0), \$r1[1] = \$r3, \$r4 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("SetGpsCoord Lat:\%s Lon:\%s", \$r1), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r2, \$r4), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$r3 = virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: android.content.Intent getIntent()$>$() (in $<$org.apache.cordova.CordovaActivity: void loadConfig()$>$)
		on Path [\$r3 = virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: android.content.Intent getIntent()$>$(), \$r4 = virtualinvoke \$r3.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), virtualinvoke \$r2.$<$org.apache.cordova.CordovaPreferences: void setPreferencesBundle(android.os.Bundle)$>$(\$r4), \$r0.$<$org.apache.cordova.CordovaPreferences: android.os.Bundle preferencesBundleExtras$>$ = \$r1, \$r0 := @this: org.apache.cordova.CordovaPreferences, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaPreferences preferences$>$, return, return, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void onStart()$>$(), staticinvoke $<$com.dynatrace.android.callback.Callback: void onStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r2.$<$com.dynatrace.android.app.LcCallbacks: void onActivityStart(android.app.Activity)$>$(\$r0), specialinvoke \$r0.$<$com.dynatrace.android.app.LcCallbacks: void logMsg(android.app.Activity,com.dynatrace.android.agent.data.LcDataConstants\-\$LcState)$>$(\$r1, \$r2), \$r5 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r6 = virtualinvoke \$r5.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), \$r4[0] = \$r6, \$r6 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("\%s ... \%s", \$r4), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r3, \$r6), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$d0 = virtualinvoke \$r1.$<$android.location.Location: double getLongitude()$>$() (in $<$com.dynatrace.android.agent.BasicSegment: void setGpsLocation(android.location.Location)$>$)
		on Path [\$d0 = virtualinvoke \$r1.$<$android.location.Location: double getLongitude()$>$(), \$r6 = staticinvoke $<$java.lang.Double: java.lang.Double valueOf(double)$>$(\$d0), \$r5[1] = \$r6, \$r7 = staticinvoke $<$java.lang.String: java.lang.String format(java.util.Locale,java.lang.String,java.lang.Object[])$>$(\$r4, "\%3.3fx\%3.3f", \$r5), \$r0.$<$com.dynatrace.android.agent.BasicSegment: java.lang.String mockDeviceLocation$>$ = \$r7, \$r9 = \$r0.$<$com.dynatrace.android.agent.BasicSegment: java.lang.String mockDeviceLocation$>$, virtualinvoke \$r8.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r9), \$r9 = virtualinvoke \$r8.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r7, \$r9), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$() (in $<$com.dynatrace.android.agent.comm.CommHandler: java.net.HttpURLConnection openConnection(java.net.URL)$>$)
		on Path [\$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$(), \$r5 = (java.net.HttpURLConnection) \$r4, return \$r5, \$r1 = virtualinvoke \$r6.$<$java.net.HttpURLConnection: java.lang.String getResponseMessage()$>$(), \$r15[1] = \$r1, \$r13 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("Response code: \%s, msg: \%s, body: \%s", \$r15), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r2, \$r13), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$r3 = virtualinvoke \$r2.$<$java.net.URL: java.net.URLConnection openConnection()$>$() (in $<$com.adobe.phonegap.push.FCMService: android.graphics.Bitmap getBitmapFromURL(java.lang.String)$>$)
		on Path [\$r3 = virtualinvoke \$r2.$<$java.net.URL: java.net.URLConnection openConnection()$>$(), \$r4 = (java.net.HttpURLConnection) \$r3, \$r5 = staticinvoke $<$com.dynatrace.android.callback.Callback: java.io.InputStream getInputStream(java.net.HttpURLConnection)$>$(\$r4), specialinvoke \$r2.$<$com.dynatrace.android.callback.ConnStateParms: void $<$init$>$(java.net.HttpURLConnection,com.dynatrace.android.callback.CbConstants\-\$WrMethod,com.dynatrace.android.callback.CbConstants\$WrStates,int)$>$(\$r0, \$r3, \$r4, 0), \$r0.$<$com.dynatrace.android.callback.ConnStateParms: java.net.HttpURLConnection conn$>$ = \$r1, return, staticinvoke $<$com.dynatrace.android.callback.Callback: void updateConnection(com.dynatrace.android.callback.ConnStateParms)$>$(\$r2), staticinvoke $<$com.dynatrace.android.callback.CallbackCore: void updateConnection(com.dynatrace.android.callback.ConnStateParms)$>$(\$r0), \$r1 = \$r0.$<$com.dynatrace.android.callback.ConnStateParms: java.net.HttpURLConnection conn$>$, \$r6 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r7 = virtualinvoke \$r6.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), \$r3[2] = \$r7, \$r7 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("\%s of \%s of \%s to \%s", \$r3), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$("caa-aCallbackCore", \$r7), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$d0 = virtualinvoke \$r0.$<$android.location.Location: double getLatitude()$>$() (in $<$com.dynatrace.android.agent.Core: int setGpsLocation(android.location.Location)$>$)
		on Path [\$d0 = virtualinvoke \$r0.$<$android.location.Location: double getLatitude()$>$(), \$r3 = staticinvoke $<$java.lang.Double: java.lang.Double valueOf(double)$>$(\$d0), \$r1[0] = \$r3, \$r4 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("SetGpsCoord Lat:\%s Lon:\%s", \$r1), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r2, \$r4), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$r1 := @parameter0: android.os.Bundle (in $<$br.gov.datasus.guardioes.MainActivity: void onCreate(android.os.Bundle)$>$)
		on Path [\$r1 := @parameter0: android.os.Bundle, specialinvoke \$r0.$<$org.apache.cordova.CordovaActivity: void onCreate(android.os.Bundle)$>$(\$r1), virtualinvoke \$r5.$<$org.apache.cordova.CordovaInterfaceImpl: void restoreInstanceState(android.os.Bundle)$>$(\$r1), \$r1 = virtualinvoke \$r1.$<$android.os.Bundle: android.os.Bundle getBundle(java.lang.String)$>$("plugin"), \$r0.$<$org.apache.cordova.CordovaInterfaceImpl: android.os.Bundle savedPluginState$>$ = \$r1, \$r0 := @this: org.apache.cordova.CordovaInterfaceImpl, \$r5 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaInterfaceImpl cordovaInterface$>$, return, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void onStart()$>$(), staticinvoke $<$com.dynatrace.android.callback.Callback: void onStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r2.$<$com.dynatrace.android.app.LcCallbacks: void onActivityStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r4.$<$com.dynatrace.android.app.LcUtility: void setActivityStateChange(android.app.Activity,com.dynatrace.android.agent.data\-.LcDataConstants\$LcState)$>$(\$r1, \$r2), \$r6 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r7 = virtualinvoke \$r6.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), \$r10[0] = \$r7, \$r7 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("\%s \%s (curr=\%s prev=\%s)", \$r10), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r4, \$r7), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$() (in $<$com.dynatrace.android.agent.comm.CommHandler: java.net.HttpURLConnection openConnection(java.net.URL)$>$)
		on Path [\$r4 = virtualinvoke \$r3.$<$java.net.URL: java.net.URLConnection openConnection()$>$(), \$r6 = (javax.net.ssl.HttpsURLConnection) \$r4, return \$r6, \$r1 = virtualinvoke \$r6.$<$java.net.HttpURLConnection: java.lang.String getResponseMessage()$>$(), \$r15[1] = \$r1, \$r13 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("Response code: \%s, msg: \%s, body: \%s", \$r15), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r2, \$r13), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]

	\item  \$d0 = virtualinvoke \$r1.$<$android.location.Location: double getLatitude()$>$() (in $<$com.dynatrace.android.agent.BasicSegment: void setGpsLocation(android.location.Location)$>$)
		on Path [\$d0 = virtualinvoke \$r1.$<$android.location.Location: double getLatitude()$>$(), \$r6 = staticinvoke $<$java.lang.Double: java.lang.Double valueOf(double)$>$(\$d0), \$r5[0] = \$r6, \$r7 = staticinvoke $<$java.lang.String: java.lang.String format(java.util.Locale,java.lang.String,java.lang.Object[])$>$(\$r4, "\%3.3fx\%3.3f", \$r5), \$r0.$<$com.dynatrace.android.agent.BasicSegment: java.lang.String mockDeviceLocation$>$ = \$r7, \$r9 = \$r0.$<$com.dynatrace.android.agent.BasicSegment: java.lang.String mockDeviceLocation$>$, virtualinvoke \$r8.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r9), \$r9 = virtualinvoke \$r8.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r7, \$r9), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r1 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int)$>$(\$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r1)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r5, \$r7) on line 19, from the following sources:
\begin{itemize}
	\item  \$r3 := @parameter1: android.content.Intent (in $<$com.adobe.phonegap.push.PushDismissedHandler: void onReceive(android.content.Context,android.content.Intent)$>$)
		on Path [\$r3 := @parameter1: android.content.Intent, \$r4 = virtualinvoke \$r3.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), virtualinvoke \$r6.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.Object)$>$(\$r4), \$r7 = virtualinvoke \$r6.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r5, \$r7)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r4, \$r6) on line 20, from the following sources:
\begin{itemize}
	\item  \$r2 := @parameter1: android.content.Intent (in $<$com.adobe.phonegap.push.BackgroundActionButtonHandler: void onReceive(android.content.Context,android.content.Intent)$>$)
		on Path [\$r2 := @parameter1: android.content.Intent, \$r3 = staticinvoke $<$android.support.v4.app.RemoteInput: android.os.Bundle getResultsFromIntent(android.content.Intent)$>$(\$r2), \$r1 = virtualinvoke \$r0.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), \$r2 = virtualinvoke \$r1.$<$android.os.Bundle: android.os.Parcelable getParcelable(java.lang.String)$>$("android.remoteinput.resultsData"), \$r1 = (android.os.Bundle) \$r2, return \$r1, \$r10 = virtualinvoke \$r3.$<$android.os.Bundle: java.lang.CharSequence getCharSequence(java.lang.String)$>$("inlineReply"), \$r4 = interfaceinvoke \$r10.$<$java.lang.CharSequence: java.lang.String toString()$>$(), virtualinvoke \$r5.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r4), \$r6 = virtualinvoke \$r5.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r4, \$r6)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$("Push\_FCMService", \$r4) on line 75, from the following sources:
\begin{itemize}
	\item  \$r1 := @parameter0: com.google.firebase.messaging.RemoteMessage (in $<$com.adobe.phonegap.push.FCMService: void onMessageReceived(com.google.firebase.messaging.RemoteMessage)$>$)
		on Path [\$r1 := @parameter0: com.google.firebase.messaging.RemoteMessage, \$r2 = virtualinvoke \$r1.$<$com.google.firebase.messaging.RemoteMessage: java.lang.String getFrom()$>$(), \$r2 = \$r0.$<$com.google.firebase.messaging.RemoteMessage: android.os.Bundle zzdp$>$, \$r1 = virtualinvoke \$r2.$<$android.os.Bundle: java.lang.String getString(java.lang.String)$>$("from"), return \$r1, virtualinvoke \$r3.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r2), \$r4 = virtualinvoke \$r3.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$("Push\_FCMService", \$r4)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$("Push\_Plugin", \$r10) on line 600, from the following sources:
\begin{itemize}
	\item  \$r2 := @parameter1: android.content.Intent (in $<$com.adobe.phonegap.push.BackgroundActionButtonHandler: void onReceive(android.content.Context,android.content.Intent)$>$)
		on Path [\$r2 := @parameter1: android.content.Intent, \$r3 = virtualinvoke \$r2.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), \$r9 = virtualinvoke \$r3.$<$android.os.Bundle: android.os.Bundle getBundle(java.lang.String)$>$("pushBundle"), staticinvoke $<$com.adobe.phonegap.push.PushPlugin: void sendExtras(android.os.Bundle)$>$(\$r9), \$r3 = staticinvoke $<$com.adobe.phonegap.push.PushPlugin: org.json.JSONObject convertBundleToJson(android.os.Bundle)$>$(\$r0), \$r7 = virtualinvoke \$r0.$<$android.os.Bundle: java.lang.Object get(java.lang.String)$>$(\$r8), \$r10 = (java.lang.String) \$r7, staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$("Push\_Plugin", \$r10)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r6, \$r11) on line 34, from the following sources:
\begin{itemize}
	\item  \$r2 := @parameter1: android.content.Intent (in $<$com.adobe.phonegap.push.BackgroundActionButtonHandler: void onReceive(android.content.Context,android.content.Intent)$>$)
		on Path [\$r2 := @parameter1: android.content.Intent, \$r3 = staticinvoke $<$android.support.v4.app.RemoteInput: android.os.Bundle getResultsFromIntent(android.content.Intent)$>$(\$r2), \$r1 = virtualinvoke \$r0.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), \$r2 = virtualinvoke \$r1.$<$android.os.Bundle: android.os.Parcelable getParcelable(java.lang.String)$>$("android.remoteinput.resultsData"), \$r1 = (android.os.Bundle) \$r2, return \$r1, \$r10 = virtualinvoke \$r3.$<$android.os.Bundle: java.lang.CharSequence getCharSequence(java.lang.String)$>$("inlineReply"), \$r4 = interfaceinvoke \$r10.$<$java.lang.CharSequence: java.lang.String toString()$>$(), virtualinvoke \$r5.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r4), \$r11 = virtualinvoke \$r5.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r6, \$r11)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r3) on line 399, from the following sources:
\begin{itemize}
	\item  \$r3 = virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: android.content.Intent getIntent()$>$() (in $<$org.apache.cordova.CordovaActivity: void loadConfig()$>$)
		on Path [\$r3 = virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: android.content.Intent getIntent()$>$(), \$r4 = virtualinvoke \$r3.$<$android.content.Intent: android.os.Bundle getExtras()$>$(), virtualinvoke \$r2.$<$org.apache.cordova.CordovaPreferences: void setPreferencesBundle(android.os.Bundle)$>$(\$r4), \$r0.$<$org.apache.cordova.CordovaPreferences: android.os.Bundle preferencesBundleExtras$>$ = \$r1, \$r0 := @this: org.apache.cordova.CordovaPreferences, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaPreferences preferences$>$, return, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void loadUrl(java.lang.String)$>$(\$r3), virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: void init()$>$(), \$r1 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaPreferences preferences$>$, interfaceinvoke \$r2.$<$org.apache.cordova.CordovaWebView: void init(org.apache.cordova.CordovaInterface,java.util.List,org.apache.cordova.Cordo\-vaPreferences)$>$(\$r3, \$r4, \$r1), \$r0.$<$org.apache.cordova.CordovaWebViewImpl: org.apache.cordova.CordovaPreferences preferences$>$ = \$r7, \$r0 := @this: org.apache.cordova.CordovaWebViewImpl, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaWebView appView$>$, \$r3 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaInterfaceImpl cordovaInterface$>$, interfaceinvoke \$r2.$<$org.apache.cordova.CordovaWebView: void init(org.apache.cordova.CordovaInterface,java.util.List,org.apache.cordova.Cordova\-Preferences)$>$(\$r3, \$r4, \$r1), \$r0.$<$org.apache.cordova.CordovaWebViewImpl: org.apache.cordova.CordovaInterface cordova$>$ = \$r5, \$r0 := @this: org.apache.cordova.CordovaWebViewImpl, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaWebView appView$>$, return, return, return, virtualinvoke \$r56.$<$br.gov.datasus.guardioes.MainActivity: void onStart()$>$(), staticinvoke $<$com.dynatrace.android.callback.Callback: void onStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r2.$<$com.dynatrace.android.app.LcCallbacks: void onActivityStart(android.app.Activity)$>$(\$r0), specialinvoke \$r0.$<$com.dynatrace.android.app.LcCallbacks: void logMsg(android.app.Activity,com.dynatrace.android.agent.data.LcDataConstants\-\$LcState)$>$(\$r1, \$r2), \$r5 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r6 = virtualinvoke \$r5.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), \$r4[0] = \$r6, \$r6 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("\%s ... \%s", \$r4), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r3, \$r6), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r3 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int,int)$>$(\$i3, \$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r3)]

	\item  \$r1 := @parameter0: android.os.Bundle (in $<$br.gov.datasus.guardioes.MainActivity: void onCreate(android.os.Bundle)$>$)
		on Path [\$r1 := @parameter0: android.os.Bundle, specialinvoke \$r0.$<$org.apache.cordova.CordovaActivity: void onCreate(android.os.Bundle)$>$(\$r1), virtualinvoke \$r5.$<$org.apache.cordova.CordovaInterfaceImpl: void restoreInstanceState(android.os.Bundle)$>$(\$r1), \$r2 = virtualinvoke \$r1.$<$android.os.Bundle: java.lang.String getString(java.lang.String)$>$("callbackService"), \$r0.$<$org.apache.cordova.CordovaInterfaceImpl: java.lang.String initCallbackService$>$ = \$r2, \$r0 := @this: org.apache.cordova.CordovaInterfaceImpl, \$r5 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaInterfaceImpl cordovaInterface$>$, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void loadUrl(java.lang.String)$>$(\$r3), virtualinvoke \$r0.$<$org.apache.cordova.CordovaActivity: void init()$>$(), \$r3 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaInterfaceImpl cordovaInterface$>$, interfaceinvoke \$r2.$<$org.apache.cordova.CordovaWebView: void init(org.apache.cordova.CordovaInterface,java.util.List,org.apache.cordova.Cordo\-vaPreferences)$>$(\$r3, \$r4, \$r1), \$r0.$<$org.apache.cordova.CordovaWebViewImpl: org.apache.cordova.CordovaInterface cordova$>$ = \$r5, \$r0 := @this: org.apache.cordova.CordovaWebViewImpl, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaWebView appView$>$, \$r3 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaInterfaceImpl cordovaInterface$>$, interfaceinvoke \$r2.$<$org.apache.cordova.CordovaWebView: void init(org.apache.cordova.CordovaInterface,java.util.List,org.apache.cordova.Cordo\-vaPreferences)$>$(\$r3, \$r4, \$r1), \$r0.$<$org.apache.cordova.CordovaWebViewImpl: org.apache.cordova.CordovaInterface cordova$>$ = \$r5, \$r0 := @this: org.apache.cordova.CordovaWebViewImpl, \$r2 = \$r0.$<$org.apache.cordova.CordovaActivity: org.apache.cordova.CordovaWebView appView$>$, return, return, return, virtualinvoke \$r0.$<$br.gov.datasus.guardioes.MainActivity: void onStart()$>$(), staticinvoke $<$com.dynatrace.android.callback.Callback: void onStart(android.app.Activity)$>$(\$r0), virtualinvoke \$r2.$<$com.dynatrace.android.app.LcCallbacks: void onActivityStart(android.app.Activity)$>$(\$r0), specialinvoke \$r0.$<$com.dynatrace.android.app.LcCallbacks: void logMsg(android.app.Activity,com.dynatrace.android.agent.data.LcDataConstants\-\$LcState)$>$(\$r1, \$r2), \$r5 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r6 = virtualinvoke \$r5.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), \$r4[0] = \$r6, \$r6 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("\%s ... \%s", \$r4), staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String)$>$(\$r3, \$r6), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r1), \$r1 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), \$r3 = virtualinvoke \$r1.$<$java.lang.String: java.lang.String substring(int,int)$>$(\$i3, \$i0), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String)$>$(\$r0, \$r3)]
\end{itemize}
\item Found a flow to sink staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r0, \$r3, \$r1) on line 405, from the following sources:
\begin{itemize}
	\item  \$r3 = virtualinvoke \$r2.$<$java.net.URL: java.net.URLConnection openConnection()$>$() (in $<$com.adobe.phonegap.push.FCMService: android.graphics.Bitmap getBitmapFromURL(java.lang.String)$>$)
		on Path [\$r3 = virtualinvoke \$r2.$<$java.net.URL: java.net.URLConnection openConnection()$>$(), \$r4 = (java.net.HttpURLConnection) \$r3, \$r5 = staticinvoke $<$com.dynatrace.android.callback.Callback: java.io.InputStream getInputStream(java.net.HttpURLConnection)$>$(\$r4), specialinvoke \$r2.$<$com.dynatrace.android.callback.ConnStateParms: void $<$init$>$(java.net.HttpURLConnection,com.dynatrace.android.callback.CbConstants\-\$WrMethod,com.dynatrace.android.callback.CbConstants\$WrStates,int)$>$(\$r0, \$r3, \$r4, 0), \$r0.$<$com.dynatrace.android.callback.ConnStateParms: java.net.HttpURLConnection conn$>$ = \$r1, return, staticinvoke $<$com.dynatrace.android.callback.Callback: void updateConnection(com.dynatrace.android.callback.ConnStateParms)$>$(\$r2), \$r2 = virtualinvoke \$r0.$<$com.dynatrace.android.callback.ConnStateParms: java.lang.String toString()$>$(), \$r3 = virtualinvoke \$r0.$<$com.dynatrace.android.callback.WebReqStateParms: java.lang.String getRequestClassName()$>$(), \$r2 = \$r0.$<$com.dynatrace.android.callback.ConnStateParms: java.net.HttpURLConnection conn$>$, \$r1 = virtualinvoke \$r0.$<$com.dynatrace.android.callback.ConnStateParms: java.lang.String getRequestClassName(java.lang.Object)$>$(\$r2), \$r2 = virtualinvoke \$r1.$<$java.lang.Object: java.lang.Class getClass()$>$(), \$r3 = virtualinvoke \$r2.$<$java.lang.Class: java.lang.String getSimpleName()$>$(), return \$r3, return \$r1, \$r1[1] = \$r3, \$r3 = staticinvoke $<$java.lang.String: java.lang.String format(java.lang.String,java.lang.Object[])$>$("\%s of \%s.\%s to \%s", \$r1), return \$r3, staticinvoke $<$com.dynatrace.android.agent.util.Utility: void zlogD(java.lang.String,java.lang.String,java.lang.Throwable)$>$("caa-aCallback", \$r2, \$r1), virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.StringBuilder append(java.lang.String)$>$(\$r3), \$r3 = virtualinvoke \$r2.$<$java.lang.StringBuilder: java.lang.String toString()$>$(), staticinvoke $<$android.util.Log: int d(java.lang.String,java.lang.String,java.lang.Throwable)$>$(\$r0, \$r3, \$r1)]
\end{itemize}		
\end{itemize}
\end{flushleft}
